Fast ion diffraction of protons on NaCl, the discovery of GIFAD

Grazing incidence fast atom diffraction (GIFAD or FAD) has become a technique to track the surface topology of crystal surface at the atomic scale. The paper retraces the events that led to the discovery of unexpected quantum behavior of keV atoms during the thesis of Patrick Rousseau in Orsay and Andreas Schueller in Berlin. In Orsay, it started by diffraction spots whereas in Berlin supernumerary rainbows were first identified at keV. Though the discovery was not anticipated, it did not take place by accident, everything was in place several years before, waiting only for an interest in neutral projectiles with a touch of curiosity.

==> refs_old.tex <==
@misc{erratum,
  title        = "{\color{purple}Erratum: Due to a bad tuning of the chopper, the H$^+$ and therefore also the H$^\circ$ beams pulse had an echo which, unfortunately, was sitting under the beginning of the second peak so that the coincidence indicates possible traces of diffraction. In this respect figure 6.10 of Ref.\cite{Rousseau_these} is erroneous. When corrected, no sign of diffraction is visible in coincidence with the second peak, as in Ref.\cite{lienemann_2011}}"
}
@misc{Natalya,
  title = "{\color{purple}N. Kalashnyk was a Post-doc in our group where she explored several perylene/{Ag} deposition schemes until diffraction could be measured with the help of M. Debiossac finishing his PhD. The work was repeated soon after on the same setup but published without any mention of their initial contribution.}"
}
@misc{MB_negative_ions,
  title        = "{\color{purple}With {Michel Barat} in 1996, we spent the last night of Beam-time at the {HCI} {(AIM)} facility in Grenoble scanning part of the periodic table present in the residual gas of the source. {We} could measure that whatever the initial charge state, grazing scattering produces negative ions whenever they exist. {W}hen packing, in the morning, {I} noticed that the tape containing our data had just been overwritten by the Linux automated backup!!!!}"
}
@misc{AIM,
  title        = "{\color{purple}We were also extremely lucky to be among the first users of the best ECR ion source at this time, the one developed in Grenoble and made available with a CEA-CNRS agreement }"
}
@misc{Chopper,
  title        = "{\color{purple}To optimize the time resolution, I decided to use edge chopping, i.e. rapididly switching a tiny beam in front of a tiny diaphragm. For this I constructed three sets of four-jaws diaphragms with Faraday cups actuated by linear stepper motors having a step resolution of 10 $\mu$m originally designed as idle gas injection in cars}"
}
@misc{Ne2,
  title        = "{\color{purple}Later, With A. Momeni and H. Khemliche, we decided to try again investigating multiply charged ions using the most simple  He$^{2+}$ and Ne$^{2+}$ ions.
We observed the 'bottle neck' paradox that more neutrals are scattered starting from Ne$^{2+}$ than from Ne$^{+}$ ions, but we could not identify the origin\cite{Momeni_these}.}"
}
@Patent{Khemliche_patent,
 author = {Khemliche, H. and Roncin, P. and Rousseau, P.},
 title={Dispositif et procédé de caracterisation de surfaces}, 
 number = {WO2008003865A2},
 url = "https://patents.google.com/patent/WO2008003865A2/fr",
 year         = 2006,
note         = "{\color{purple}H. Khemliche was the one who decided to pattent but he did not contribute to any part of the setup nor to the acquisition and analysis software and he was opposed to the decision of investigating neutrals {H$^\circ$ on NaCl} that led to the discovery of GIFAD.}"
}//howpublished = "\url{https://patents.google.com/patent/WO2008003865A2/fr}",

@misc{Henkel,
  title        = "{\color{purple}See Ref.\cite{Henkel_94} for adaptation to atoms on evanescent waves above a dielectric surface, Ref.\cite{Debiossac_PRA_2014} for adaptation to GIFAD, Refs.\cite{brandt1968channeling,krause1986rainbow} for the channeling of MeV ions in crystals and Refs.\cite{danailov_1991scattering,danailov2001deduction,farias_2004_pronounced,zugarramurdi_2012_transition,muzas_2016_diffraction} for independent rediscoveries of the decoupling effect also named axial surface channeling approximation (ASCA).}"
}

@article{rau1973measurement,
  title={Measurement of predominant electron spin orientation at single crystal surfaces of ferromagnetic nickel},
  author={Rau, C and Sizmann, R},
  journal={Physics Letters A},
  volume={43},
  number={4},
  pages={317--318},
  year={1973},
  publisher={Elsevier}
}
@article {Andreev_2002,
	author = {Andreev, E.A.},
	title = {Quantum and classical characteristics of glancing scattering of fast atoms on the surface of a crystal},
	volume = {76},
	year = {2002},
	Pages = {164-169},
	doi = {10.1126/science.1098490},
	Journal = {Russ. J. Phys. Chem. A}
}//Russian Journal of Physical Chemistry A  
%URL = {https://elibrary.ru/item.asp?id=13413403},
@phdthesis{xiang_these,
  TITLE = {{Interaction of fast ({keV}) hydrogen ions/atoms with surfaces : diffraction and negative ion formation}},
  AUTHOR = {Xiang, Yang},
  URL = {https://theses.hal.science/tel-00863479},
  NUMBER = {2012PA112161},
  SCHOOL = {{Univ. Paris Sud 11}},
  YEAR = {2012},
  note = "dirigée par P. Roncin",
}
@PhDThesis{Villette_these,
title = {Etude exp\'{e}rimentale de l'int\'{e}raction rasante d'atomes et d'ions sur des surfaces isolantes},
author = {J\'{e}r\^{o}me Villette},
school = {Univ. Paris Sud 11},
note = "dirigée par P. Roncin",
year = {2000},
url = {https://tel.archives-ouvertes.fr/tel-00106816/document}
}
@PHDTHESIS{Momeni_these,
url = "http://www.theses.fr/2003PA066459",
title = "Etude expérimentale des processus multi-électroniques lors de collisions d'ions en incidence rasante sur une surface de {LiF}(001)",
author = "Momeni, Anouchah",
year = "2003",
note = "dirigée par P.Roncin, Paris 6.",
url = "http://www.theses.fr/2003PA066459/document",
}

@PHDTHESIS{szila1997,
url = "http://www.theses.fr/1997PA112101",
title = "Etude experimentale de l'interaction ion multicharge - surface",
author = "SZILAGYI, SZABOLCS-ZOLTAN",
year = "1997",
note = "dirigée par M.Barat, Paris 11 1997",
}

@PHDTHESIS{Atana_these,
url = "http://www.theses.fr/1999PA066022",
title = "Interaction de proton avec une surface de fluorure de lithium : correlations entre la perte d'energie et l'emission electronique",
author = "Atanas, Jean-Pierre",
year = "1999",
note = "dirigée par M.Barat, Paris 6 1999"
}
@article{bocan2018gifad,
  title={Gifad for he/{KCl} (001). structure in the pattern for< 110> incidence as a measure of the projectile-cation interaction},
  author={Bocan, Gisela Anah{\'\i} and Gravielle, Maria Silvia},
  journal={NIM-B},
  volume={421},
  pages={1--6},
  year={2018},
  publisher={Elsevier}
}
@PHDTHESIS{Rousseau_these,
url = "https://theses.hal.science/tel-00106727",
title = "Collisions rasantes d'ions ou d'atomes sur les surfaces : de l'échange de charge à la diffraction atomique",
author = "Rousseau, Patrick",
year = "2007",
note = "dirigée par P. Roncin",
school = "Univ. Paris Sud 11"
}
//http://www.theses.fr/2006PA112140/document
@article{Rousseau_2008,
	doi = {10.1088/1742-6596/133/1/012013},
	url = {https://doi.org/10.1088%2F1742-6596%2F133%2F1%2F012013},
	year = 2008,
	month = {oct},
	publisher = {{IOP} Publishing},
	volume = {133},
	pages = {012013},
	author = {Patrick Rousseau and Hocine Khemliche and Nenad Bundaleski and Pierre Soulisse and Anouchah Momeni and Philippe Roncin},
	title = {Surface analysis with grazing incidence fast atom diffraction ({GIFAD})},
	journal = {J. Phys. Conf. Ser.},
}
@article{bundaleski2011decoherence,
  title={Decoherence in fast atom diffraction from surfaces},
  author={Bundaleski, N and Soulisse, P and Momeni, Anouchah and Khemliche, H and Roncin, P},
  journal={NIM-B},
  volume={269},
  number={11},
  pages={1216--1220},
  year={2011},
  publisher={Elsevier},
 doi={10.1016/j.nimb.2010.12.056}
}
@PHDTHESIS{soulisse_2011,
title = "Développement d'un dispositif expérimental pour la diffraction d'atomes rapides et étude de surfaces d'isolants ioniques",
author = "Soulisse, Pierre",
year = "2011",
note = "dirigée par P.Roncin",
school = "Univ. Paris Sud 11",
url = "http://www.theses.fr/2011PA112118/document"
}
@PHDTHESIS{debiossac_these,
title = "Diffraction d’atomes rapides sur surfaces : des résonances de piégeage à la dynamique de croissance par épitaxie",
author = "Debiossac, Maxime",
year = "2014",
note = "dirigée par P.Roncin",
school = "Univ. Paris Sud 11",
url = "http://www.theses.fr/2014PA112384/document"
}

@phdthesis{Meyer_2016,
author = {Meyer, Eric},
title = {Strukturuntersuchungen an Oxidkristalloberflächen mittels der streifenden Streuung schneller Atome},
school = {Humboldt-Universität zu Berlin, Mathematisch-Naturwissenschaftliche Fakultät},
year = {2016},
doi = {http://dx.doi.org/10.18452/17442}
}
@article{winter1991recent,
  title={Recent advances in understanding particle-induced electron emission from metal surfaces},
  author={Winter, HP and Aumayr, F and Lakits, G},
  journal={NIM-B},
  volume={58},
  number={3-4},
  pages={301--308},
  year={1991},
  publisher={Elsevier}
}
@article{wilhelm2017interatomic,
  title={Interatomic coulombic decay: the mechanism for rapid deexcitation of hollow atoms},
  author={Wilhelm, Richard A and Gruber, Elisabeth and Schwestka, Janine and Kozubek, Roland and Madeira, Teresa I and Marques, Jos{\'e} P and Kobus, Jacek and Krasheninnikov, Arkady V and Schleberger, Marika and Aumayr, Friedrich},
  journal={Physical review letters},
  volume={119},
  number={10},
  pages={103401},
  year={2017},
  publisher={APS}
}
@article{fujii1993layer,
  title={Layer-by-layer growth of GaAs studied by glancing angle scattering of fast ions},
  author={Fujii, Yoshikazu and Narumi, Kazumasa and Kimura, Kenji and Mannami, Michi-hiko and Hashimoto, Toyoyuki and Ogawa, Kiyoshi and Ohtani, Fumihiko and Yoshida, Tamio and Asari, Masatoshi},
  journal={Applied physics letters},
  volume={63},
  number={15},
  pages={2070--2072},
  year={1993},
  publisher={American Institute of Physics}
}
@article{iwai1982cross,
  title={Cross sections for one-electron capture by highly stripped ions of {B, C, N, O, F, Ne, and S} from {He} below 1 {keV}/amu},
  author={Iwai, T and Kaneko, Y and Kimura, M and Kobayashi, N and Ohtani, S and Okuno, K and Takagi, S and Tawara, H and Tsurubuchi, S},
  journal={Phys. Rev. A},
  volume={26},
  number={1},
  pages={105},
  year={1982},
  publisher={APS}
}
@article{datz1978resonant,
  title={Resonant coherent excitation of channeled ions},
  author={Datz, S and Moak, CD and Crawford, OH and Krause, HF and Dittner, PF and Del Campo, J Gomez and Biggerstaff, JA and Miller, PD and Hvelplund, P and Knudsen, H},
  journal={Physical Review Letters},
  volume={40},
  number={13},
  pages={843},
  year={1978},
  publisher={APS}
}
@article{khemliche2009electron,
  title={Electron excitations in grazing diffraction of fast He on a {Ag} (110) surface. A tribute to {H}annspeter {W}inter},
  author={Khemliche, H and Bundaleski, N and Soulisse, P and Roncin, P},
  journal={NIM-B},
  volume={267},
  doi={doi:10.1016/j.nimb.2008.11.009},
  number={4},
  pages={620--623},
  year={2009},
  publisher={Elsevier}
}
@article{Manson_PRB_2008,
  title = {Theory of grazing incidence diffraction of fast atoms and molecules from surfaces},
  author = {Manson, J. R. and Khemliche, Hocine and Roncin, Philippe},
  journal = {Phys. Rev. B},
  volume = {78},
  issue = {15},
  pages = {155408},
  numpages = {15},
  year = {2008},
  doi = {10.1103/PhysRevB.78.155408}
}  //month = {Oct},
  publisher = {American Physical Society},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.78.155408}

@inproceedings{young1832bakerian,
  title={The Bakerian lecture. Experiments and calculations relative to physical optics},
  author={Young, Thomas},
  booktitle={Philos. Trans. R. Soc. London},
  pages={1--16},
  year={1804}, 
}//  number={1},pages={131--132},organization={The Royal Society London}
@inproceedings{Descartes_1637,
  title={Les météores},
  author={Descartes, René},
  year={1637}, 
}
@article{newton2014letter,
  title={{A letter of Mr. Isaac Newton containing his new theory about light and colors: sent by the author to the publisher from Cambridge}},
  author={Newton, Isaac},
  journal={Philos. Trans. R. Soc. London},
  volume={6},
  pages={3075--3087},
  year={1671},
}// Professor of the Mathematicks in the University of Cambridge; number={80},publisher={The Royal Society London} , in order to be communicated to the R. Society
@inproceedings{kapitza1933reflection,
  title={The reflection of electrons from standing light waves},
  author={Kapitza, PL and Dirac, PAM},
  booktitle={Math. Proc. Camb. Philos. Soc.},
  volume={29},
  pages={297--300},
  year={1933},
  organization={Cambridge University Press}
}// number ={2},
@article{schuller2005interatomic,
  title={Interatomic potentials from rainbow scattering of {keV} noble gas atoms under axial surface channeling},
  author={Sch{\"u}ller, A and Wethekam, S and Mertens, A and Maass, K and Winter, H and G{\"a}rtner, K},
  journal={NIM-B},
  volume={230},
  number={1-4},
  pages={172--177},
  year={2005},
  publisher={Elsevier}
}
@article{khemliche2009grazing,
  title={Grazing incidence fast atom diffraction: An innovative approach to surface structure analysis},
  author={Khemliche, H and Rousseau, Patrick and Roncin, P and Etgens, Victor H and Finocchi, Fabio},
  journal={Applied Physics Letters},
  volume={95},
  number={15},
  year={2009},
  publisher={AIP Publishing},
  DOI = {10.1063/1.3246162}
}

@article{estermann_1930,
  title={Beugung von molekularstrahlen},
  author={Estermann, Immanuel and Stern, Otto},
  journal={Z. Phys.},
  volume={61},
  number={1-2},
  pages={95--125},
  year={1930},
  publisher={Springer}
}
@article{knauer_1929reflexion,
  title={{\"U}ber die reflexion von molekularstrahlen},
  author={Knauer, F and Stern, Otto},
  journal={Z. Phys.},
  volume={53},
  number={11-12},
  pages={779--791},
  year={1929},
  publisher={Springer}
}
@article{winter1979nuclear,
  title={Nuclear polarized $^{7}${Li} and $^{14}${N} ions via ion beam surface interaction at grazing incidence},
  author={Winter, H and Andr{\"a}, HJ},
  journal={Z. Phys. A Atoms and Nuclei},
  volume={291},
  number={1},
  pages={5--9},
  year={1979},
  publisher={Springer}
}
@article{winter1983band,
  title={Band structure effects in high energy ion beam surface interaction at grazing incidence},
  author={Winter, H and Zimny, R and Schirmacher, A and Becker, B and Andr{\"a}, HJ and Fr{\"o}hling, R},
  journal={Z. Phys. A Atoms and Nuclei},
  volume={311},
  pages={267--280},
  year={1983},
  publisher={Springer}
}
@article{hoekstra1990state,
  title={State-selective charge transfer in slow collisions of {C}$^{4+}$ with {H} and {H}$_2$},
  author={Hoekstra, R and Beijers, JPM and Schlatmann, AR and Morgenstern, R and de Heer, FJ},
  journal={Phys. Rev. A},
  volume={41},
  number={9},
  pages={4800},
  year={1990},
  publisher={APS}
}
@article{toennies_2011otto,
  title={Otto Stern (1888--1969): The founding father of experimental atomic physics},
  author={Toennies, J Peter and Schmidt-B{\"o}cking, Horst and Friedrich, Bretislav and Lower, Julian CA},
  journal={Annalen der Physik},
  volume={523},
  number={12},
  pages={1045--1070},
  year={2011},
  publisher={Wiley Online Library}
}
@article{STOLTERFOHT_1971,
Author = {Stolterfoht, N},
Title = {ANGULAR AND ENERGY DISTRIBUTION OF ELECTRONS PRODUCED BY 200-500 ke{V}
   PROTONS IN GASES .1. HELIUM},
Journal = {Z. Phys.},
Year = {1971},
Volume = {248},
Number = {1},
Pages = {81+},
DOI = {10.1007/BF01394837},
ISSN = {0044-3328},
Unique-ID = {WOS:A1971K906700008},
}
@article{muller1977scaling,
  title={Scaling of cross sections for multiple electron transfer to highly charged ions colliding with atoms and molecules},
  author={M{\"u}ller, Alfred and Salzborn, Erhard},
  journal={Physics Letters A},
  volume={62},
  number={6},
  pages={391--394},
  year={1977},
  publisher={Elsevier}
}
@article{ULLRICH_1986,
Author = {Kelbch, S and Ullrich, J and Rauch, W and Schmidt-Bocking, H and
   Horbatsch, M and Dreeizler, RM and Hagmann, S and Anholt, R and
   Schachter, AS and Müller, A and Richard, P and Stoller, C and Cocke, CL
   and Mann, R and Meyerhof, WE and others},
Title = {MULTIPLE IONIZATION OF {Ne, Ar, Kr} AND {I} BY NEARLY RELATIVISTIC {U} IONS},
Journal = {J. Phys. B.},
Year = {1986},
Volume = {19},
Number = {2},
Pages = {L47-L52},
DOI = {10.1088/0022-3700/19/2/002},
ISSN = {0953-4075},
ResearcherID-Numbers = {Muller, Alfred/A-3548-2009
   },
ORCID-Numbers = {Muller, Alfred/0000-0002-0030-6929
   Horbatsch, Marko/0000-0002-6163-7502},
Unique-ID = {WOS:A1986AZD6700002},
}%Month = {JAN 28},and Rasmussen, JD

@article{nelson1963penetration,
  title={The penetration of energetic ions through the open channels in a crystal lattice},
  author={Nelson, RS and Thompson, MW},
  journal={Philosophical Magazine},
  volume={8},
  number={94},
  pages={1677--1690},
  year={1963},
  publisher={Taylor \& Francis}
}//Channeling
@article{brandt1968channeling,
  title={Channeling in crystals},
  author={Brandt, Werner},
  journal={Scientific American},
  url = {https://www.jstor.org/stable/10.2307/24926002},
  volume={218},
  number={3},
  pages={90--101},
  year={1968},
  publisher={JSTOR}
}//Channeling
@article{krause1986rainbow,
  title={Rainbow effect in axial ion channeling},
  author={Krause, HF and Datz, S and Dittner, PF and del Campo, J Gomez and Miller, PD and Moak, CD and Neskovi{\'c}, N and Pepmiller, PL},
  journal={Phys. Rev. B},
  volume={33},
  number={9},
  pages={6036},
  year={1986},
  publisher={APS}
}//Channeling
@article{Rousseau_2010,
Author = {Holm, A. I. S. and Zettergren, H. and Johansson, H. A. B. and Seitz, F.
   and Rosen, S. and Schmidt, H. T. and Lawicki, A. and Rangama, J. and
   Rousseau, P. and Capron, M. and Maisonny, R. and Adoui, L. and Mery, A.
   and Manil, B. and Huber, B. A. and Cederquist, H.},
Title = {Ions Colliding with Cold Polycyclic Aromatic Hydrocarbon Clusters},
Journal = {Phys. Rev. Lett},
Year = {2010},
Volume = {105},
Number = {21},
url = {https://dx.doi.org/10.1103/PhysRevLett.105.213401},
}//Month = {NOV 19},
Article-Number = {213401},
DOI = {10.1103/PhysRevLett.105.213401},
ISSN = {0031-9007},
EISSN = {1079-7114},
Unique-ID = {WOS:000284407400012},
doi = {10.1088/0031-8949/1997/T73/057},
url = {https://dx.doi.org/10.1088/0031-8949/1997/T73/057},
@article{aumayr1993emission,
  title={Emission of electrons from a clean gold surface induced by slow, very highly charged ions at the image charge acceleration limit},
  author={Aumayr, F and Kurz, H and Schneider, D and Briere, MA and McDonald, JW and Cunningham, CE and Winter, HP},
  journal={Phys. Rev. Lett},
  volume={71},
  number={12},
  pages={1943},
  year={1993},
  publisher={APS}
}
@article{fujii1988surface,
  title={Surface channeling of {MeV} {He}$^+$ ions on a {SnTe} single crystal},
  author={Fujii, Y and Kimura, K and Hasegawa, M and Suzuki, M and Susuki, Y and Mannami, M},
  journal={NIM-B},
  volume={33},
  number={1-4},
  pages={405--408},
  year={1988},
  publisher={Elsevier}
}
@article{snowdon1988observation,
  title={Observation of skipping motion in small-angle ion-surface scattering},
  author={Snowdon, KJ and O'connor, DJ and MacDonald, RJ},
  journal={Physical review letters},
  volume={61},
  number={15},
  pages={1760},
  year={1988},
  publisher={APS}
}
@article{winter1990grazing,
  title={Grazing scattering of fast protons at a clean {W}(100) surface},
  author={Winter, H and Remillieux, J and Poizat, JC},
  journal={NIM-B},
  volume={48},
  number={1-4},
  pages={382--385},
  year={1990},
  publisher={Elsevier}
}
@article{briand1984observation,
  title={Observation of the {KLL} dielectronic recombination process in highly stripped argon ions},
  author={Briand, JP and Charles, P and Arianer, J and Laurent, H and Goldstein, C and Dubau, J and Loulergue, M and Bely-Dubau, F},
  doi = {10.1103/PhysRevLett.52.617},
  journal={Phys. Rev. Lett.},
  volume={52},
  number={8},
  pages={617},
  year={1984},
  publisher={APS},
  note={{\color{purple}I was starting my {PhD} in the same hall and I was asked to keep an eye and 'stabilize' the voltage of the electrons injected in the {EBIS}. {I} was pleased to read that {I} deserved a few Volts stability over several hours.}}
}
@article{Martin_1985,
Author = {Buchet, JP and Buchet-Pouliac, MC and Denis, A and Desesquelles, J and
   Druetta, M and Martin, S and Grandin, JP and Husson, X and Lesteven, I},
Title = {BEAM-FOIL STUDY OF THE 2S$^2$2P$^5$3l and 2s$^2$p$^6$3l Configurations of {FeXVII}},
Journal = {Phys. Scr.},
Year = {1985},
Volume = {31},
Number = {5},
Pages = {364-368},
DOI = {10.1088/0031-8949/31/5/010},
ISSN = {0281-1847},
Unique-ID = {WOS:A1985ALR3700010},
}
@article{Roncin_1986,
	doi = {10.1088/0022-3735/19/1/005},
	year = 1986,
	month = {jan},
	publisher = {{IOP} Publishing},
	volume = {19},
	number = {1},
	pages = {37--40},
	author = {P Roncin and H Laurent and M Barat},
	title = {An electrostatic spectrometer for a simultaneous analysis of energy and scattering angle},
    url = {https://doi.org/10.1088%2F0022-3735%2F19%2F1%2F005},
	journal = {J. Phys. E: Sci. Instr.}
}%url = {https://doi.org/10.1088%2F0022-3735%2F19%2F1%2F005},
@article{ Henkel_94,
	author = {{C. Henkel} and {J.-Y. Courtois} and {A. Aspect}},
	title = {Atomic diffraction by a thin phase grating},
	DOI= "10.1051/jp2:1994242",
	url= "https://doi.org/10.1051/jp2:1994242",
	journal = {J. Phys. II France},
	year = 1994,
	volume = 4,
	number = 11,
	pages = "1955-1974"
}%
@article{Morosov_1996,
author = {Morosov,V A. and Kalinin,A. and Szilagyi,Z. and Barat,M. and Roncin,P. },
title = {2$\pi$ spectrometer: A new apparatus for the investigation of ion surface interaction},
journal = {Rev. Sci. Instrum.},
volume = {67},
number = {6},
pages = {2163-2170},
year = {1996},
doi = {10.1063/1.1147031},
}%URL = {https://doi.org/10.1063/1.1147031}

@article{poole_1973_NaCl,
  title={A photoelectron study of the alkali chlorides},
  author={Poole, RT and Jenkin, JG and Leckey, RCG and Liesegang, J},
  journal={Chemical Physics Letters},
  volume={22},
  number={1},
  pages={101--104},
  year={1973},
  publisher={Elsevier}
}
@article{morosov1997correlation,
  title={Correlation between projectile Auger electrons and slow secondary electrons emitted in collisions of highly charged ions with an insulator surface},
  author={Morosov, VA and Gaboriaud, MN and Barat, M and Roncin, P},
  journal={NIM-B},
  volume={125},
  number={1-4},
  pages={167--169},
  year={1997},
  publisher={Elsevier}
}
@article{roncin_2002_F,
  title={Evidence for {F$^-$} formation by simultaneous double-electron capture during scattering of {F$^+$} from a {LiF} (001) surface},
  author={Roncin, P and Borisov, AG and Khemliche, H and Momeni, A and Mertens, A and Winter, H},
  journal={Phys. Rev. Lett},
  doi={10.1103/PhysRevLett.89.043201 },
  volume={89},
  number={4},
  pages={043201},
  year={2002},
  publisher={APS}
}
@article{borisov1997theory,
  title={Theory of negative-ion conversion of neutral atoms in grazing scattering from alkali halide surfaces},
  author={Borisov, AG and Sidis, V},
  journal={Phys. Rev. B},
  volume={56},
  number={16},
  pages={10628},
  year={1997},
  publisher={APS},
  doi = {10.1103/PhysRevB.56.10628}
}
@article{Debiossac_PRA_2014,
  title = {Atomic diffraction under oblique incidence: An analytical expression},
  author = {Debiossac, Maxime and Roncin, Philippe},
  journal = {Phys. Rev. A},
  volume = {90},
  issue = {5},
  pages = {054701},
  numpages = {5},
  year = {2014},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.90.054701},
}%url = {https://link.aps.org/doi/10.1103/PhysRevA.90.054701}

@article{flechard1997state,
  title={State-selective double-electron capture in low-velocity collisions studied by recoil-ion momentum spectroscopy},
  author={Flechard, X and Duponchel, S and Adoui, L and Cassimi, A and Roncin, P and Hennecart, D},
  journal={J. Phys. B},
  volume={30},
  number={16},
  pages={3697},
  year={1997},
  publisher={IOP Publishing}
}
@article{Bernard_1997,
doi = {10.1088/0031-8949/1997/T73/057},
url = {https://dx.doi.org/10.1088/0031-8949/1997/T73/057},
year = {1997},
number = {T73},
pages = {190},
author = {Jérôme Bernard and  Li Chen and  Alain Denis and  Jean Désesquelles and  Serge Martin and  Michel Barat and  Philippe Roncin},
title = {Double Rydberg states in stabilized triple capture in bare ions ({Z} = 6-10) on rare gas target collisions},
journal = {Phys. Scr.}
}%month = {jan},volume = {1997},
@article{miret2012classical,
  title={Classical theory of atom--surface scattering: The rainbow effect},
  author={Miret-Art{\'e}s, Salvador and Pollak, Eli},
  journal={Surface Science Reports},
  volume={67},
  number={7-8},
  pages={161--200},
  year={2012},
  publisher={Elsevier}
}
@article{Avrin1994,
   author = {William F. Avrin and Robert P. Merrill},
   doi = {10.1016/0039-6028(94)90498-7},
   issn = {00396028},
   issue = {1-2},
   journal = {Surface Science},
   month = {5},
   pages = {269-280},
   title = {Simplified analysis of helium scattering: supernumerary rainbows from a soft, corrugated potential},
   volume = {311},
   year = {1994},
}
@article{garibaldi1975quantum,
  title={Quantum theory of atom-surface scattering: Diffraction and rainbow},
  author={Garibaldi, U and Levi, AC and Spadacini, R and Tommei, GE},
  journal={Surface Science},
  volume={48},
  number={2},
  pages={649--675},
  year={1975},
  publisher={Elsevier}
}
@article{pan2022setup,
  title={A setup for grazing incidence fast atom diffraction},
  author={Pan, Peng and Rad, Jaafar Najafi and Roncin, Philippe},
  journal={Rev. Sci. Instrum.},
  doi={10.1063/5.0099269},
  volume={93},
  number={9},
  year={2022},
  publisher={AIP Publishing}
}
@article{Winter_PSS_2011,
title = "Fast atom diffraction during grazing scattering from surfaces",
journal = "Progress in Surface Science",
volume = "86",
number = "9",
pages = "169 - 221",
year = "2011",
issn = "0079-6816",
doi = "https://doi.org/10.1016/j.progsurf.2011.07.001",
url = "http://www.sciencedirect.com/science/article/pii/S0079681611000311",
author = {H. Winter and A. Sch\"uller},
}
@article{Pollak_2015,
author = {Pollak,E.  and Miret-Art\'{e}s,S.},
title = {Second-Order Semiclassical Perturbation Theory for Diffractive Scattering from a Surface},
journal = {J. Phys. Chem. C},
volume = {119},
number = {12},
pages = {14532},
year = {2015},
doi = {doi: 10.1021/jp509500v},
URL = {https://doi.org/10.1021/jp509500v},
eprint = {https://pubs.acs.org/doi/abs/10.1021/jp509500v}
}
@article{rousseau2005neutralization,
  title={Neutralization of noble gas ions on ionic insulators: Auger neutralization or double-electron capture},
  author={Rousseau, Patrick and Gugiu, M and Khemliche, H and Roncin, P},
  journal={NIM-B},
  volume={230},
  number={1-4},
  pages={361--368},
  year={2005},
  publisher={Elsevier}
}
@article{rousseau2007auger,
  title={Auger rates on {NaCl(001)}, effect of the final state and modeling via an effective length},
  author={Rousseau, Patrick and Khemliche, H and Roncin, P},
  journal={NIM-B},
  volume={258},
  number={1},
  pages={13--17},
  year={2007},
  publisher={Elsevier}
}
@article{auth1998threshold,
  title={Threshold in the stopping of slow protons scattered from the surface of a wide-band-gap insulator},
  author={Auth, C and Mertens, A and Winter, H and Borisov, A},
  journal={Phys. Rev. Lett},
  volume={81},
  number={22},
  pages={4831},
  year={1998},
  publisher={APS}
}
@article{mertens_2000,
  title={Energy transfer from fast atomic projectiles to a crystal lattice under channeling conditions},
  author={Mertens, A and Winter, H},
  journal={Phys. Rev. Lett},
  volume={85},
  number={13},
  pages={2825},
  year={2000},
  publisher={APS}
}
@article{Roncin_1999,
  title = {Energy Loss of Low Energy Protons on {LiF(100)}: Surface Excitation and ${H}^{-}$ Mediated Electron Emission},
  author = {Roncin, P. and Villette, J. and Atanas, J. P. and Khemliche, H.},
  journal = {Phys. Rev. Lett.},
  volume = {83},
  issue = {4},
  pages = {864--867},
  numpages = {0},
  year = {1999},
  month = {jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.83.864},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.83.864},
  note={{\color{purple}When writing the paper, H. Khemliche arrived in the group and was offered to be on the author's list as a welcome sign.}}
}
@article{villette_2000_cal,
  title={Calibration of a multiple microchannel plate detectors system by $\alpha$-induced secondary electrons},
  author={Villette, J and Barat, M and Roncin, P},
  journal={Rev. Sci. Instrum.},
  volume={71},
  number={6},
  pages={2367--2370},
  year={2000},
  publisher={American Institute of Physics}
}
@article{arnau1997,
  title={Interaction of slow multicharged ions with solid surfaces},
  author={Arnau, Antonio and Aumayr, F and Echenique, PM and Grether, M and Heiland, W and Limburg, J and Morgenstern, R and Roncin, P and Schippers, S and Schuch, R and others},
  journal={Surf. Sci. Reports},
  volume={27},
  number={4-6},
  pages={113--239},
  year={1997},
  publisher={Elsevier}
}
@article{khemliche_1999_Lshell,
  title={L-shell filling of {N}$^{6+}$  and {O}$^{7+}$ ions from a clean and {LiF}-covered {Au} (111) surface},
  author={Khemliche, H and Schlath{\"o}lter, T and Hoekstra, R and Morgenstern, R},
  journal={Phys. Rev. A},
  volume={60},
  number={5},
  pages={3800},
  year={1999},
  publisher={APS}
}
@article{khemliche_1999_hollow,
  title={Hollow atom dynamics on thin films},
  author={Khemliche, H and Laulh{\'e}, C and Hoekstra, S and Hoekstra, R and Morgenstern, R},
  journal={Phys. Scr.},
  volume={1999},
  number={T80A},
  pages={66},
  year={1999},
  publisher={IOP Publishing}
}
@article{khemliche2001electron,
  title={Electron bihole complex formation in neutralization of {Ne}$^+$ on {LiF} (001)},
  author={Khemliche, H and Villette, J and Borisov, AG and Momeni, A and Roncin, P},
  journal={Phys. Rev. Lett},
  doi={10.1103/PhysRevLett.86.5699},
  volume={86},
  number={25},
  pages={5699},
  year={2001},
  publisher={APS}
}
@article{Villette_2000,
  title = {Subsurface-Channeling-Like Energy Loss Structure of the Skipping Motion on an Ionic Crystal},
  author = {Villette, J. and Borisov, A. G. and Khemliche, H. and Momeni, A. and Roncin, P.},
  journal = {Phys. Rev. Lett.},
  volume = {85},
  issue = {15},
  pages = {3137--3140},
  numpages = {0},
  year = {2000},
doi = {10.1103/PhysRevLett.85.3137},
  //month = {Oct},
  publisher = {American Physical Society},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.85.3137}
}
@article{dirsyte2009surface,
  title={Surface termination of the {NdGaO$_3$} (110)},
  author={Dirsyte, R and Schwarzkopf, J and Wagner, G and Lienemann, J and Busch, M and Winter, H and Fornari, R},
  journal={Appl. Surf. Sci.},
  volume={255},
  number={20},
  pages={8685--8687},
  year={2009},
  publisher={Elsevier}
}
@article{lienemann_2011,
  title={Coherence during scattering of fast {H} atoms from a {LiF} (001) surface},
  author={Lienemann, J and Sch{\"u}ller, A and Blauth, D and Seifert, J and Wethekam, S and Busch, M and Maass, K and Winter, H},
  journal={Phys. Rev. Lett},
  volume={106},
  number={6},
  pages={067602},
  year={2011},
  publisher={APS},
  doi = {10.1103/PhysRevLett.106.067602},
}
@article{roncin2017elastic,
  title={Elastic and inelastic diffraction of fast atoms, {Debye-Waller} factor, and M{\"o}ssbauer-{Lamb-Dicke} regime},
  author={Roncin, Philippe and Debiossac, Maxime},
  journal={Phys. Rev. B},
  volume={96},
  number={3},
  pages={035415},
  year={2017},
doi={10.1103/PhysRevB.96.035415},
  publisher={APS}
}
@article{mertens2000energy,
  title={Energy transfer from fast atomic projectiles to a crystal lattice under channeling conditions},
  author={Mertens, A and Winter, H},
  journal={Physical review letters},
  volume={85},
  number={13},
  pages={2825},
  year={2000},
  publisher={APS}
}

@book{friedrich_2021_molecular,
  title={Molecular Beams in Physics and Chemistry: From Otto Stern's Pioneering Exploits to Present-Day Feats},
  author={Friedrich, Bretislav and Schmidt-B{\"o}cking, Horst},
  year={2021},
  publisher={Springer Nature}
}
@article{Schuller_2007,
  title = {Diffraction of Fast Atomic Projectiles during Grazing Scattering from a {LiF}(001) Surface},
  author = {Sch\"uller, A. and Wethekam, S. and Winter, H.},
  journal = {Phys. Rev. Lett.},
  volume = {98},
  issue = {1},
  pages = {016103},
  numpages = {4},
  year = {2007},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.98.016103},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.98.016103}
}//month = {Jan},
@article{schuller2010rumpling,
  title={Rumpling of {LiF} (001) surface from fast atom diffraction},
  author={Sch{\"u}ller, A and Wethekam, Stephan and Blauth, D and Winter, H and Aigner, Florian and Simonovi{\'c}, N and Solleder, B and Burgd{\"o}rfer, Joachim and Wirtz, Ludger},
  journal={Physical Review A},
  volume={82},
  number={6},
  pages={062902},
  year={2010},
  publisher={APS},
   DOI={10.1103/PhysRevA.82.062902}
}
@article{niehus1993low,
  title={Low-energy ion scattering at surfaces},
  author={Niehus, Horst and Heiland, Werner and Taglauer, Edmund},
  journal={Surf. Sci. Reports},
  volume={17},
  number={4-5},
  pages={213--303},
  year={1993},
  publisher={Elsevier}
}
@article{mertens2002excitation,
  title={Excitation vs electron emission near the kinetic thresholds for grazing impact of hydrogen atoms on {LiF} (001)},
  author={Mertens, A and Lederer, S and Maass, K and Winter, H and St{\"o}ckl, J and Winter, HP and Aumayr, F},
  journal={Phys. Rev. B},
  volume={65},
  number={13},
  pages={132410},
  year={2002},
  publisher={APS}
}
@article{khemliche2002exciton,
  title={Exciton and trion formation during neutralization of {Ne$^+$} at a {LiF} (001) surface},
  author={Khemliche, H and Borisov, AG and Momeni, A and Roncin, P},
  journal={NIM-B},
  volume={191},
  number={1-4},
  pages={221--225},
  year={2002},
  publisher={Elsevier}
}
@article{borisov2003f,
  title={{F$^-$} formation via simultaneous two-electron capture during grazing scattering of {F$^+$} ions from a {LiF} (001) surface},
  author={Borisov, AG and Sidis, V and Roncin, P and Momeni, A and Khemliche, H and Mertens, A and Winter, H},
  journal={Phys. Rev. B},
  volume={67},
  number={11},
  pages={115403},
  doi={10.1103/PhysRevLett.89.043201},
  year={2003},
  publisher={APS}
}
@article{Rousseau_2007,
  title = {Quantum Scattering of Fast Atoms and Molecules on Surfaces},
  author = {Rousseau, P. and Khemliche, H. and Borisov, A. G. and Roncin, P.},
  journal = {Phys. Rev. Lett.},
  volume = {98},
  issue = {1},
  pages = {016104},
  numpages = {4},
  year = {2007},
  //month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.98.016104},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.98.016104}
}
@article{barat1990single,
  title={Single and double electron capture by {C}$^{4+}$ ions colliding with helium target},
  author={Barat, M and Roncin, P and Guillemot, L and Gaboriaud, MN and Laurent, H},
  journal={J. Phys. B},
  volume={23},
  number={16},
  pages={2811},
  year={1990},
  doi={10.1088/0953-4075/23/16/022},
  publisher={IOP Publishing}
}
@article{borisov1999evidence,
  title={Evidence for the stopping of slow ions by excitations of optical phonons in insulators},
  author={Borisov, AG and Mertens, A and Winter, H and Kazansky, AK},
  journal={Phys. Rev. Lett},
  volume={83},
  number={25},
  pages={5378},
  year={1999},
  publisher={APS},
  doi = {10.1103/PhysRevLett.83.5378}
}
@article{auth1995image,
  title={Image charge acceleration of multicharged ions in front of the surface of an insulator},
  author={Auth, Ch and Hecht, T and Igel, T and Winter, H},
  journal={Phys. Rev. Lett},
  volume={74},
  number={26},
  pages={5244},
  year={1995},
  publisher={APS}
}
@article{Atkinson_2014,
author = {Atkinson,P.  and Eddrief,M.  and Etgens,V. H.  and Khemliche,H.  and Debiossac,M.  and Momeni,A.  and Mulier,M.  and Lalmi,B.  and Roncin,P. },
title = {Dynamic grazing incidence fast atom diffraction during molecular beam epitaxial growth of {GaAs}},
journal = {Applied Physics Letters},
volume = {105},
number = {2},
pages = {021602},
year = {2014},
doi = {10.1063/1.4890121},
URL = { https://doi.org/10.1063/1.4890121}
}//eprint = { https://doi.org/10.1063/1.4890121}
@article{Debiossac_2017,
title = "Fast atom diffraction inside a molecular beam epitaxy chamber, a rich combination",
journal = "Appl. Surf. Sci.",
volume = "391",
pages = "53 - 58",
year = "2017",
doi = "https://doi.org/10.1016/j.apsusc.2016.02.157",
author = "M. Debiossac and P. Atkinson and A. Zugarramurdi and M. Eddrief and F. Finocchi and V.H. Etgens and A. Momeni and H. Khemliche and A.G. Borisov and P. Roncin",
//note = "European Conference on Surface Science 2015",
//issn = "0169-4332",
//url = "http://www.sciencedirect.com/science/article/pii/S016943321630335X",
}

@article{Debiossac_PRB_2014,
  title = {Combined experimental and theoretical study of fast atom diffraction on the ${\ensuremath{\beta}}_{2}(2\ifmmode\times\else\texttimes\fi{}4)$ reconstructed {GaAs}(001) surface},
  author = {Debiossac, M. and Zugarramurdi, A. and Khemliche, H. and Roncin, P. and Borisov, A. G. and Momeni, A. and Atkinson, P. and Eddrief, M. and Finocchi, F. and Etgens, V. H.},
  journal = {Phys. Rev. B},
  volume = {90},
  issue = {15},
  pages = {155308},
  numpages = {13},
  year = {2014},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.90.155308},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.90.155308}
}
@article{debiossac2014transient,
  title={Transient quantum trapping of fast atoms at surfaces},
  author={Debiossac, M and Zugarramurdi, A and Lunca-Popa, P and Momeni, A and Khemliche, H and Borisov, AG and Roncin, P},
  journal={Physical Review Letters},
  doi = {10.1103/PhysRevLett.112.023203},
  volume={112},
  number={2},
  pages={023203},
  year={2014},
  publisher={APS}
}//url = {https://link.aps.org/doi/10.1103/PhysRevLett.112.023203},
@article{lennard_1936diffraction,
  title={Diffraction and selective adsorption of atoms at crystal surfaces},
  author={Lennard-Jones, John Edward and Devonshire, AF},
  journal={Nature},
  volume={137},
  number={3478},
  pages={1069--1070},
  year={1936},
  publisher={Nature Publishing Group UK London}
}
@article{frisch_1933anomalien,
  title={Anomalien bei der spiegelnden Reflexion und Beugung von Molekularstrahlen an Kristallspaltfl{\"a}chen. {I}},
  author={Frisch, R and Stern, O},
  journal={Z. Phys.},
  volume={84},
  number={7-8},
  pages={430--442},
  year={1933},
  publisher={Springer}
}
@article{villette_1999grazing,
  title={Grazing collision of {keV} protons on {LiF} correlation between energy loss and electron emission},
  author={Villette, J and Atanas, JP and Khemliche, H and Barat, M and Morosov, V and Roncin, P},
  journal={NIM-B},
  volume={157},
  number={1-4},
  pages={92--97},
  year={1999},
  publisher={Elsevier}
}
@article{kohrbruck1992auger,
  title={Auger-electron emission from slow, highly charged ions interacting with solid Cu targets},
  author={K{\"o}hrbr{\"u}ck, R and Sommer, K and Biersack, JP and Bleck-Neuhaus, J and Schippers, S and Roncin, P and Lecler, D and Fremont, F and Stolterfoht, N},
  journal={Phys. Rev. A},
  volume={45},
  number={7},
  pages={4653},
  year={1992},
  publisher={APS}
}
@article{kohrbruck1991electron,
  title={Electron emission in collisions of slow, highly charged ions with gases and solid surfaces},
  author={K{\"o}hrbr{\"u}ck, R and Lecler, D and Fremont, F and Roncin, P and Sommer, K and Zouros, TJM and Bleck-Neuhaus, J and Stolterfoht, N},
  journal={NIM-B},
  volume={56},
  pages={219--222},
  year={1991},
  publisher={Elsevier}
}
@article{stolterfoht2002transmission,
  title={Transmission of 3 {keV Ne} $^{7+}$ ions through nanocapillaries etched in polymer foils: Evidence for capillary guiding},
  author={Stolterfoht, N and Bremer, J-H and Hoffmann, V and Hellhammer, R and Fink, D and Petrov, A and Sulik, B},
  journal={Phys. Rev. Lett},
  volume={88},
  number={13},
  pages={133201},
  year={2002},
  publisher={APS}
}

@article{cassimi2009imaging,
  title={Imaging dynamics of charge-auto-organisation in glass capillaries},
  author={Cassimi, Amine and Maunoury, Laurent and Muranaka, Tomoko and Huber, B and Dey, Kalpana R and Lebius, Henning and Leli{\`e}vre, Daniel and Ramillon, Jean-Marc and Been, Thierry and Ikeda, T and others},
  journal={NIM-B},
  volume={267},
  number={4},
  pages={674--677},
  year={2009},
  publisher={Elsevier}
}
@article{aigner2008suppression,
  title={Suppression of decoherence in fast-atom diffraction at surfaces},
  author={Aigner, Florian and Simonovi{\'c}, N and Solleder, B and Wirtz, Ludger and Burgd{\"o}rfer, Joachim},
  journal={Physical Review Letters},
  volume={101},
  number={25},
  pages={253201},
  year={2008},
  publisher={APS},
  DOI= {10.1103/PhysRevLett.101.253201}
}
@article{cassimi2012dynamics,
  title={Dynamics of charge evolution in glass capillaries for 230-{keV Xe} $^{23+}$ ions},
  author={Cassimi, A and Ikeda, T and Maunoury, L and Zhou, CL and Guillous, S and Mery, A and Lebius, H and Benyagoub, A and Grygiel, C and Khemliche, H and others},
  journal={Phys. Rev. A},
  volume={86},
  number={6},
  pages={062902},
  year={2012},
  publisher={APS}
}
@article{tamtogl_2017_electron,
  title={Electron-phonon coupling and surface Debye temperature of {$Bi_2 Te_3$} (111) from helium atom scattering},
  author={Tamt{\"o}gl, Anton and Kraus, Patrick and Avidor, Nadav and Bremholm, Martin and Hedegaard, Ellen MJ and Iversen, Bo B and Bianchi, Marco and Hofmann, Philip and Ellis, John and Allison, William and others},
  journal={Phys. Rev. B},
  volume={95},
  number={19},
  pages={195401},
  year={2017},
  publisher={APS}
}
@article{kelsall_2021_ultrafast,
  title={Ultrafast diffusion at the onset of growth: O/Ru (0001)},
  author={Kelsall, Jack and Townsend, Peter SM and Ellis, John and Jardine, Andrew P and Avidor, Nadav},
  journal={Phys. Rev. Lett},
  volume={126},
  number={15},
  pages={155901},
  year={2021},
  publisher={APS}
}
@article{jardine_2009_helium,
  title={Helium-3 spin-echo: Principles and application to dynamics at surfaces},
  author={Jardine, AP and Hedgeland, H and Alexandrowicz, G and Allison, W and Ellis, J},
  journal={Progress in Surf. Sci.},
  volume={84},
  number={11-12},
  pages={323--379},
  year={2009},
  publisher={Elsevier}
}
@article{Lupone_2018,
title = "A large area high resolution imaging detector for fast atom diffraction",
journal = "NIM-B",
volume = "427",
pages = "95 - 99",
year = "2018",
issn = "0168-583X",
doi = "10.1016/j.nimb.2018.04.030",
url = "http://www.sciencedirect.com/science/article/pii/S0168583X18302751",
author = "Sylvain Lupone and Pierre Soulisse and Philippe Roncin",
keywords = "Fast atom diffraction, Reflexion high energy electron diffraction, Imaging detector"
}
@article{debiossac_2021_grazing,
  title={Grazing incidence fast atom diffraction, similarities and differences with thermal energy atom scattering (TEAS)},
  author={Debiossac, Maxime and Pan, Peng and Roncin, Philippe},
  journal={Physical Chemistry Chemical Physics},
  volume={23},
  number={13},
  pages={7615--7636},
  year={2021},
  doi={10.1039/d0cp05476c},
  publisher={Royal Society of Chemistry}
}
@article{zugarramurdi_2012_transition,
  title={Transition from fast to slow atom diffraction},
  author={Zugarramurdi, Asier and Borisov, Andrei G},
  journal={Phys. Rev. A},
  volume={86},
  number={6},
  pages={062903},
  year={2012},
  publisher={APS},
  DOI={10.1103/PhysRevA.86.062903}
}
@article{zugarramurdi2013surface,
  title={Surface-grating deflection of fast atom beams},
  author={Zugarramurdi, A and Debiossac, M and Lunca-Popa, P and Alarc{\'o}n, LS and Momeni, A and Khemliche, H and Roncin, P and Borisov, AG},
  journal={Physical Review A},
  volume={88},
  number={1},
  pages={012904},
  year={2013},
  publisher={APS},
  doi={1050-2947/2013/88(1)/012904}
}
@article{aigner_2008,
  title={Suppression of decoherence in fast-atom diffraction at surfaces},
  author={Aigner, F and Simonovi{\'c}, N and Solleder, B and Wirtz, Ludger and Burgd{\"o}rfer, Joachim},
  journal={Phys. Rev. Lett},
  volume={101},
  number={25},
  pages={253201},
  year={2008},
  publisher={APS}
}
@article{jardine_2004_ultrahigh,
  title={Ultrahigh-resolution spin-echo measurement of surface potential energy landscapes},
  author={Jardine, Andrew P and Dworski, Shechar and Fouquet, Peter and Alexandrowicz, Gil and Riley, David J and Lee, Gabriel YH and Ellis, John and Allison, William},
  journal={Science},
  volume={304},
  number={5678},
  pages={1790--1793},
  year={2004},
  doi = {10.1126/science.1098490},
  publisher={American Association for the Advancement of Science}
}
@article{indelicato1992relativistic,
  title={Relativistic effects, correlation, and {QED} corrections on {K}$\alpha$ transitions in medium to very heavy atoms},
  author={Indelicato, Paul and Lindroth, E},
  journal={Phys. Rev. A},
  volume={46},
  number={5},
  pages={2426},
  year={1992},
  publisher={APS}
}
@article{king2022optical,
  title={An optical atomic clock based on a highly charged ion},
  author={King, Steven A and Spie{\ss}, Lukas J and Micke, Peter and Wilzewski, Alexander and Leopold, Tobias and Benkler, Erik and Lange, Richard and Huntemann, Nils and others},
  journal={Nature},
  volume={611},
  number={7934},
  pages={43--47},
  year={2022},
  publisher={Nature Publishing Group UK London}
}%and Surzhykov, Andrey and Yerokhin, Vladimir A 
@article{farias_1998_atomic,
  title={Atomic beam diffraction from solid surfaces},
  author={Farias, Daniel and Rieder, Karl-Heinz},
  journal={Reports on Progress in Physics},
  volume={61},
  number={12},
  pages={1575},
  year={1998},
  publisher={IOP Publishing}
}
@article{muzas_2016_diffraction,
  title={Diffraction of {H} from {LiF}(001): From slow normal incidence to fast grazing incidence},
  author={Muzas, AS and Gatti, Fabien and Mart{\'\i}n, Fernando and D{\'\i}az, C},
  journal={NIM-B},
  volume={382},
  pages={49--53},
  year={2016},
  publisher={Elsevier},
  doi={10.1016/j.nimb.2016.04.031}
}
@article{roncin1987transfer,
  title={Transfer ionization in collisions involving multiply charged ions at low {keV} energy},
  author={Roncin, P and Gaboriaud, MN and Barat, M and Laurent, H},
  journal={E.P.L.},
  volume={3},
  number={1},
  pages={53},
  year={1987},
  publisher={IOP Publishing}
}//EuroPhysics Letters
@article{debiossac_2020_refraction,
  title={Refraction of fast {Ne} atoms in the attractive well of a {LiF}(001) surface},
  author={Debiossac, Maxime and Roncin, Philippe and Borisov, AG},
  journal={The Journal of Physical Chemistry Letters},
  volume={11},
  number={12},
  pages={4564--4569},
  year={2020},
  doi={10.1021/acs.jpclett.0c01157},
  publisher={ACS Publications}
}
@article{seifert2010diffraction,
  title={Diffraction of fast atoms during grazing scattering from the surface of an ultrathin silica film on Mo (112)},
  author={Seifert, J and Sch{\"u}ller, A and Winter, H and W{\l}odarczyk, R and Sauer, J and Sierka, M},
  journal={Physical Review B},
  volume={82},
  number={3},
  pages={035436},
  year={2010},
  publisher={APS}
}

@article{seifert2011transition,
  title={Transition from axial to planar surface channeling for fast atom diffraction},
  author={Seifert, J and Sch{\"u}ller, A and Winter, H and G{\"a}rtner, K},
  journal={NIM-B},
  volume={269},
  number={11},
  pages={1212--1215},
  year={2011},
  publisher={Elsevier},
  doi={10.1016/j.nimb.2010.11.050}
}
@article{farias_2004_pronounced,
  title={Pronounced out-of-plane diffraction of {H$_2$} molecules from a {Pd} (111) surface},
  author={Far{\i}as, D and D{\i}az, C and Nieto, P and Salin, A and Mart{\i}n, F},
  journal={Chem. phys. lett.},
  volume={390},
  number={1-3},
  pages={250--255},
  year={2004},
  publisher={Elsevier},
 DOI = {10.1016/j.cplett.2004.03.151}
}

@article{busch_2013_diffraction,
  title={Diffraction of fast H atoms during grazing scattering from an {Al} $\{$sub 2$\}$ O $\{$sub 3$\}$(1 1 2 $\{$sup{\={}}$\}$ 0) surface},
  author={Busch, M and Seifert, J and Meyer, E and Winter, H and others},
  journal={NIM-B},
  volume={317},
  year={2013}
}
@article{busch_2012_evidence,
  title={Evidence for longitudinal coherence in fast atom diffraction},
  author={Busch, M and Seifert, J and Meyer, E and Winter, H},
  journal={Phys. Rev. B},
  volume={86},
  number={24},
  pages={241402},
  year={2012},
  publisher={APS},
  doi={1098-0121/2012/86(24)/241402(4)}
}
@article{feiten2015surface,
  title={Surface structure of {V}$_2${O}$_3$(0001) revisited},
  author={Feiten, Felix E and Seifert, Jan and Paier, Joachim and Kuhlenbeck, Helmut and Winter, Helmut and Sauer, Joachim and Freund, Hans-Joachim},
  journal={Physical Review Letters},
  volume={114},
  number={21},
  pages={216101},
  year={2015},
  doi = {10.1103/PhysRevLett.114.216101},
  publisher={APS}
}//Phys. Rev. Lett. Physical Review Letters
@article{Seifert_2009,
  title = {Evidence for {2D}-Network Structure of Monolayer Silica Film on {Mo}(112)},
  author = {Seifert, J. and Blauth, D. and Winter, H.},
  journal = {Phys. Rev. Lett.},
  volume = {103},
  issue = {1},
  pages = {017601},
  numpages = {4},
  year = {2009},
  month = {jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.103.017601},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.103.017601}
}
@article{Seifert_2013,
Author = {Seifert, J. and Busch, M. and Meyer, E. and Winter, H.},
Title = {{Surface Structure of Alanine on Cu(110) Studied by Fast Atom Diffraction}},
Journal = {{Phys. Rev. Lett.}},
Year = {{2013}},
Volume = {{111}},
Number = {{13}},
pages = {137601},
month = {{SEP 25}},
DOI = {{10.1103/PhysRevLett.111.137601}},
Article-Number = {{137601}},
ISSN = {{0031-9007}},
EISSN = {{1079-7114}},
Unique-ID = {{ISI:000325362500019}},
URL = {https://doi.org/10.1103/PhysRevLett.111.137601}
}
@article{cartry_2017alternative,
  title={Alternative solutions to caesium in negative-ion sources: a study of negative-ion surface production on diamond in H2/D2 plasmas},
  author={Cartry, Gilles and Kogut, Dmitry and Achkasov, Kostiantyn and Layet, Jean-Marc and Farley, Thomas and Gicquel, Alix and Achard, Jocelyn and Brinza, Ovidiu and Bieber, Thomas and Khemliche, Hocine and others},
  journal={New Journal of Physics},
  volume={19},
  number={2},
  pages={025010},
  year={2017},
  publisher={IOP Publishing}
}
@article{borisov_1992h,
  title={H$^-$ formation by electron capture in hydrogen-{Al} (111) collisions: perturbative and nonperturbative approaches},
  author={Borisov, AG and Teillet-Billy, D and Gauyacq, JP},
  journal={Surf. Sci.},
  volume={278},
  pages={99--110},
  year={1992},
  publisher={Elsevier},
  DOI = {10.1016/0039-6028(92)90586-U}
}%number={1-2},
@article{Schueller2008Supernumerary,
  title = {Supernumerary Rainbows in the Angular Distribution of Scattered Projectiles for Grazing Collisions of Fast Atoms with a {LiF}(001) Surface},
  author = {Sch\"uller, A. and Winter, H.},
  journal = {Phys. Rev. Lett.},
  volume = {100},
  issue = {9},
  pages = {097602},
  numpages = {4},
  year = {2008},
doi = {10.1103/PhysRevLett.100.097602}
}//url = {https://link.aps.org/doi/10.1103/PhysRevLett.100.097602}
@article{borisov_1993singlet,
  title={Singlet-to-triplet conversion in low energy metastable helium-metal surface collisions},
  author={Borisov, AG and Teillet-Billy, D and Gauyacq, JP},
  journal={Surf. Sci.},
  volume={284},
  number={3},
  pages={337--348},
  year={1993},
  publisher={Elsevier},
  DOI = {10.1016/0039-6028(93)90504-D}
}
@article{Lalmi_2012,
	doi = {10.1088/0953-8984/24/44/442002},
	url = {https://doi.org/10.1088%2F0953-8984%2F24%2F44%2F442002},
	year = 2012,
	month = {oct},
	publisher = {{IOP} Publishing},
	volume = {24},
	number = {44},
	pages = {442002},
	author = {B Lalmi and H Khemliche and A Momeni and P Soulisse and P Roncin},
	title = {High resolution imaging of superficial mosaicity in single crystals using grazing incidence fast atom diffraction},
	journal = {J. Phys. Condens. Matter},
}
@article{bundaleski2008grazing,
  title={Grazing incidence diffraction of {keV} helium atoms on a {Ag (110)} surface},
  author={Bundaleski, N and Khemliche, H and Soulisse, P and Roncin, P},
  journal={Physical Review Letters},
  dou={10.1103/PhysRevLett.101.177601},
  volume={101},
  number={17},
  pages={177601},
  year={2008},
  publisher={APS},
  doi={10.1103/PhysRevLett.101.177601}
}//url={https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.101.177601},
@article{busch2009fast,
  title={Fast atom diffraction at metal surface},
  author={Busch, M and Sch{\"u}ller, A and Wethekam, S and Winter, H},
  journal={Surface science},
  volume={603},
  number={3},
  pages={L23--L26},
  year={2009},
  publisher={Elsevier},
doi={10.1016/j.susc.2008.12.021}
}
@article{ Cooper_edge,
Author = {Murty, MVR and Cooper, BH},
Title = {Instability in molecular beam epitaxy due to fast edge diffusion and
   corner diffusion barriers},
Journal = {Phys. Rev. Lett},
Year = {1999},
Volume = {83},
Number = {2},
Pages = {352-355},
Month = {JUL 12},
DOI = {10.1103/PhysRevLett.83.352},
ISSN = {0031-9007},
Unique-ID = {WOS:000081358900028},
}
@article{ Cooper_CT,
Author = {Kimmel, GA and Cooper, BH},
Title = {DYNAMICS OF RESONANT CHARGE-TRANSFER IN LOW-ENERGY ALKALI-METAL-ION
   SCATTERING},
Journal = {Phys. Rev. B},
Year = {1993},
Volume = {48},
Number = {16},
Pages = {12164-12177},
Month = {OCT 15},
DOI = {10.1103/PhysRevB.48.12164},
ISSN = {0163-1829},
ResearcherID-Numbers = {Kimmel, Greg A/H-5355-2018},
ORCID-Numbers = {Kimmel, Greg A/0000-0003-4447-2440},
Unique-ID = {WOS:A1993ME60100079},
}
@article{dirubio1996energy,
  title={Energy transfer, trapping, and the interaction potential in hyperthermal {Na}$^+$ scattering from {Cu} (001)},
  author={DiRubio, CA and McEachern, RL and McLean, JG and Cooper, BH},
  journal={Phys. Rev. B},
  volume={54},
  number={12},
  pages={8862},
  year={1996},
  publisher={APS}
}
@article{ Cooper_Xray_PRL,
Author = {Murty, MVR and Curcic, T and Judy, A and Cooper, BH and Woll, AR and
   Brock, JD and Kycia, S and Headrick, RL},
Title = {X-ray scattering study of the surface morphology of {A}u(111) during {Ar}$^+$
   ion irradiation},
Journal = {Phys. Rev. Lett.},
Year = {1998},
Volume = {80},
Number = {21},
Pages = {4713-4716},
Month = {MAY 25},
DOI = {10.1103/PhysRevLett.80.4713},
ISSN = {0031-9007},
ResearcherID-Numbers = {Kycia, Stefan/HTS-3389-2023
   Brock, Joel/AAZ-3439-2020
   },
ORCID-Numbers = {Kycia, Stefan/0000-0003-0039-2318
   Woll, Arthur/0000-0001-8925-2199},
Unique-ID = {WOS:000073794600026},
}
@article{donets1998historical,
  title={Historical review of electron beam ion sources},
  author={Donets, Evgeni D},
  doi={10.1063/1.1148642},
  journal={Rev. Sci. Instrum.},
  volume={69},
  number={2},
  pages={614--619},
  year={1998},
  publisher={American Institute of Physics},
note={{\color{purple}{In} an {EBIS}, ions are confined in {UHV} and exposed to an electron beam of defined energy. {After} a cooking time, the ions reach an equilibrium charge state and can be extracted.}}
}
@book{geller2018electron,
  title={Electron cyclotron resonance ion sources and ECR plasmas},
  author={Geller, Richard},
  year={2018},
  publisher={Routledge},
note={{\color{purple}In {ECR}, a plasma in high vacuum is confined in a magnetic bottle so that a resonnance sheet is present where electrons can absorb a few {100 W} of microwave power heating the nano-gram of gas to million degrees. {The} electron energy distribution is broad but a {DC} extraction produces almost {mA} of ion current which needs to be filtrered in q/m.}}
}
@article{knudsen1984experimental,
  title={An experimental investigation of double ionisation of helium atoms in collisions with fast, fully stripped ions},
  author={Knudsen, H and Andersen, LH and Hvelplund, P and Astner, G and Cederquist, H and Danared, H and Liljeby, L and Rensfelt, K-G},
  journal={J. Phys. B.},
  volume={17},
  number={17},
  pages={3545},
  year={1984},
  publisher={IOP Publishing}
}//Danared, H and Liljeby, L and Rensfelt, K-G
@article{kilgus1992high,
  title={High-resolution measurement of dielectronic recombination of lithiumlike {Cu}$^{26+}$},
  author={Kilgus, G and Habs, D and Schwalm, D and Wolf, A and Badnell, NR and M{\"u}ller, A},
  journal={Phys. Rev. A},
  volume={46},
  number={9},
  pages={5730},
  year={1992},
  publisher={APS}
}
@article{thomas2011double,
  title={The double electrostatic ion ring experiment: A unique cryogenic electrostatic storage ring for merged ion-beams studies},
  author={Thomas, Richard D and Schmidt, Henning T and Andler, Guillermo and Bj{\"o}rkhage, Mikael and Blom, Mikael and Br{\"a}nnholm, Lars and B{\"a}ckstr{\"o}m, E and others},
  journal={Rev. Sci. Instrum.},
  volume={82},
  number={6},
  year={2011},
  publisher={AIP Publishing}
}// and Danared, H{\aa}kan
@article{villette1999grazing,
  title={Grazing collision of {keV} protons on {LiF} correlation between energy loss and electron emission},
  author={Villette, J and Atanas, JP and Khemliche, H and Barat, M and Morosov, V and Roncin, P},
  journal={NIM-B},
  volume={157},
  number={1-4},
  pages={92--97},
  year={1999},
  publisher={Elsevier}
}
@article{manil2003highly,
  title={Highly charged clusters of fullerenes: charge mobility and appearance sizes},
  author={Manil, B and Maunoury, L and Huber, BA and Jensen, J and Schmidt, HT and Zettergren, H and Cederquist, H and Tomita, S and Hvelplund, P},
  journal={Physical review letters},
  volume={91},
  number={21},
  pages={215504},
  year={2003},
  publisher={APS}
}
@article{cederquist2000electronic,
  title={Electronic response of C 60 in slow collisions with highly charged ions},
  author={Cederquist, H and Fardi, A and Haghighat, K and Langereis, A and Schmidt, HT and Schwartz, SH and Levin, JC and Sellin, IA and Lebius, H and Huber, B and others},
  journal={Phys. Rev. A},
  volume={61},
  number={2},
  pages={022712},
  year={2000},
  publisher={APS}
}
@article{bernard2008tabletop,
  title={A “tabletop” electrostatic ion storage ring: Mini-Ring},
  author={Bernard, J and Montagne, G and Br{\'e}dy, R and Terpend-Ordaci{\`e}re, B and Bourgey, A and Kerleroux, M and Chen, Li and Schmidt, HT and Cederquist, Henrik and Martin, S},
  journal={Rev. Sci. Instrum.},
  volume={79},
  number={7},
  year={2008},
  publisher={AIP Publishing}
}
@article{barat1992multiple,
  title={Multiple electron capture by highly charged ions at {keV} energies},
  author={Barat, M and Roncin, Ph},
  journal={J. Phys. B},
  volume={25},
  number={10},
  pages={2205},
  year={1992},
  publisher={IOP Publishing}
}

@article{borisov_1996_diabatic,
  title={Diabatic energy level confluence: the mechanism of negative ion conversion of neutral atoms in grazing scattering from insulator surfaces},
  author={Borisov, AG and Sidis, V and Winter, H},
  journal={Phys. Rev. Lett},
  volume={77},
  number={9},
  pages={1893},
  year={1996},
  publisher={APS},
 DOI = {10.1103/PhysRevLett.77.1893}
}
@article{maazouz1996h,
  title={H$^-$ formation in the scattering of hydrogen ions on an Al surface},
  author={Maazouz, M and Baragiola, R and Borisov, A and Esaulov, VA and Lacombe, S and Gauyacq, JP and Guillemot, L and Teillet-Billy, D},
  journal={Surf. Sci.},
  volume={364},
  number={2},
  pages={L568--L574},
  year={1996},
  publisher={Elsevier}
}
@article{borisov_1993energy,
  title={Energy shift and broadening of {H} levels in front of a metal surface},
  author={Borisov, AG and Teillet-Billy, D and Gauyacq, JP},
  journal={NIM-B},
  volume={78},
  number={1-4},
  pages={49--55},
  year={1993},
  publisher={Elsevier},
  DOI = {10.1016/0168-583X(93)95775-Z}
}
@article{hecht_2000role,
  title={Role of the {2D} surface state continuum and projected band gap in charge transfer in front of a {Cu} (111) surface},
  author={Hecht, T and Winter, H and Borisov, AG and Gauyacq, JP and Kazansky, AK},
  journal={Phys. Rev. Lett},
  volume={84},
  number={11},
  pages={2517},
  year={2000},
  publisher={APS},
DOI = {10.1103/PhysRevLett.84.2517}
}

@article{hecht_1998auger,
  title={Auger transition rates for the neutralization of {He}$^+$ ions in front of an aluminium surface},
  author={Hecht, T and Winter, H and Borisov, AG},
  journal={Surf. Sci.},
  volume={406},
  number={1-3},
  pages={L607--L613},
  year={1998},
  publisher={Elsevier}
}
@article{deutscher_1999formation,
  title={Formation of negative ions from fluorine projectiles scattered off a {MgO} (100) surface: Theory},
  author={Deutscher, Stefan A and Borisov, Andrei G and Sidis, Victor},
  journal={Phys. Rev. A},
  volume={59},
  number={6},
  pages={4446},
  year={1999},
  publisher={APS}
}
@article{borisov_1999bandgap,
  title={Resonant charge transfer in ion--metal surface collisions: Effect of a projected band gap in the H$^-$ {Cu} (111) system},
  author={Borisov, AG and Kazansky, AK and Gauyacq, JP},
  journal={Phys. Rev. B},
  volume={59},
  number={16},
  pages={10935},
  year={1999},
  publisher={APS}
}
@article{borisov_1996shifted,
  title={Resonant charge transfer in grazing scattering of alkali-metal ions from an {Al} (111) surface},
  author={Borisov, AG and Teillet-Billy, D and Gauyacq, JP and Winter, H and Dierkes, G},
  journal={Phys. Rev. B},
  volume={54},
  number={23},
  pages={17166},
  year={1996},
  publisher={APS}
}
@article{geerlings1985h,
  title={H$^-$ Formation in proton-metal collisions},
  author={Geerlings, JJC and Van Amersfoort, PW and Kwakman, LF Tz and Granneman, EHA and Los, J and Gauyacq, JP},
  journal={Surf. Sci.},
  volume={157},
  number={1},
  pages={151--161},
  year={1985},
  publisher={Elsevier}
}
@article{Kalashnyk_2016,
title = "Atom beam triangulation of organic layers at 100 meV normal energy: self-assembled perylene on {Ag}(110) at room temperature",
journal = "Appl. Surf. Sci.",
volume = "364",
pages = "235 - 240",
year = "2016",
issn = "0169-4332",
doi = "https://doi.org/10.1016/j.apsusc.2015.12.134",
url = "http://www.sciencedirect.com/science/article/pii/S0169433215031396",
author = "Nataliya Kalashnyk and Hocine Khemliche and Philippe Roncin",
keywords = "Organic layer on surface, On-line monitoring of growth and organisation"
}
@article{niehof1990experimental,
  title={Experimental realisation of low-energy surface channeling},
  author={Niehof, A and Heiland, W},
  journal={NIM-B},
  volume={48},
  number={1-4},
  pages={306--310},
  year={1990},
  publisher={Elsevier}
}
@article{johnson2022safari,
  title={SAFARI--A low and hyperthermal energy ion scattering simulation},
  author={Johnson, PR and Sosolik, CE},
  journal={Computer Physics Communications},
  volume={280},
  pages={108479},
  year={2022},
  publisher={Elsevier}
}
@article{roncin_1987TI,
  title={Transfer ionization in collisions involving multiply charged ions at low {keV} energy},
  author={Roncin, P and Gaboriaud, MN and Barat, M and Laurent, H},
  journal={EuroPhysics Letters},
  volume={3},
  number={1},
  pages={53},
  year={1987},
  publisher={IOP Publishing}
}
@article{danailov_1991scattering,
  title={Scattering of energetic beams at glancing incidence from crystal surfaces: a molecular dynamics simulation},
  author={Danailov, D and Rechtien, J-H and Snowdon, KJ},
  journal={Surf. Sci.},
  volume={259},
  number={3},
  pages={359--370},
  year={1991},
  publisher={Elsevier}
}
@article{danailov2001deduction,
  title={Deduction of the {He}--{Fe} interaction potential in {eV}-range from experimental data by computer simulation in grazing ion-surface scattering: {Row-model}},
  author={Danailov, Daniel and Pfandzelter, Rupert and Igel, Thomas and Winter, Helmut and G{\"a}rtner, Konrad},
  journal={NIM-B},
  volume={180},
  number={1-4},
  pages={265--273},
  year={2001},
  publisher={Elsevier},
  DOI = {10.1016/S0168-583X(01)00427-X}
}
@article{Rabalais_1997composition,
  title={Composition and structure of the Al2O3 $\{$0001$\}$-(1$\times$ 1) surface},
  author={Ahn, J and Rabalais, JW},
  journal={Surf. Sci.},
  volume={388},
  number={1-3},
  pages={121--131},
  year={1997},
  publisher={Elsevier}
}
@article{grizzi1990tofsars,
  title={Time-of-flight scattering and recoiling spectrometer (TOF-SARS) for surface analysis},
  author={Grizzi, O and Shi, M and Bu, H and Rabalais, JW},
  journal={Rev. Sci. Instrum.},
  volume={61},
  number={2},
  pages={740--752},
  year={1990},
  publisher={American Institute of Physics}
}
@article{masson1989application,
  title={Application of direct recoil spectrometry to determination of the saturation coverage of ethylene on {Pt} (111)},
  author={Masson, Francois and Sass, Craig S and Grizzi, Oscar and Rabalais, J Wayne},
  journal={Surf. Sci.},
  volume={221},
  number={1-2},
  pages={299--316},
  year={1989},
  publisher={Elsevier}
}
@article{Taglauer_1993leis,
  title={Low-energy ion scattering at surfaces},
  author={Niehus, Horst and Heiland, Werner and Taglauer, Edmund},
  journal={Surf. Sci. Reports},
  volume={17},
  number={4-5},
  pages={213--303},
  year={1993},
  publisher={Elsevier}
}
@article{primetzhofer2008strength,
  title={Strength of the interatomic potential derived from angular scans in LEIS},
  author={Primetzhofer, D and Markin, SN and Draxler, M and Beikler, R and Taglauer, E and Bauer, P},
  journal={Surf. Sci.},
  volume={602},
  number={17},
  pages={2921--2926},
  year={2008},
  publisher={Elsevier}
}
@article{delcorte1997tof,
  title={ToF-SIMS analyses of polystyrene and dibenzanthracene: evidence for fragmentation and metastable decay processes in molecular secondary ion emission},
  author={Delcorte, Arnaud and Segda, BG and Bertrand, Patrick},
  journal={Surf. Sci.},
  volume={381},
  number={1},
  pages={18--32},
  year={1997},
  publisher={Elsevier}
}
@article{hatke_1997RCE,
  title={Surface Channeling Experiments at 20 MeV and Resonant Coherent Excitation of N 6+ Ions},
  author={Hatke, N and Dirska, M and Grether, M and Luderer, E and Robin, A and N{\"a}rmann, A and Heiland, W},
  journal={Phys. Rev. Lett},
  volume={79},
  number={18},
  pages={3395},
  year={1997},
  publisher={APS}
}
@article{auth_1997resonant,
  title={Resonant coherent excitation of fast hydrogen atoms in front of a {LiF}(001) surface},
  author={Auth, C and Mertens, A and Winter, H and Borisov, AG and de Abajo, FJ Garcia},
  journal={Phys. Rev. Lett},
  volume={79},
  number={22},
  pages={4477},
  year={1997},
  publisher={APS}
}
@article{juaristi1999charge,
  title={Charge state dependence of the energy loss of slow ions in metals},
  author={Juaristi, JI and Arnau, A and Echenique, PM and Auth, C and Winter, H},
  journal={Phys. Rev. Lett},
  volume={82},
  number={5},
  pages={1048},
  year={1999},
  publisher={APS}
}
@article{maazouz1998electron,
  title={Electron capture and loss in the scattering of hydrogen and oxygen ions on a {Si} surface},
  author={Maazouz, M and Guillemot, L and Esaulov, VA and O'Connor, DJ},
  journal={Surf. Sci.},
  volume={398},
  number={1-2},
  pages={49--59},
  year={1998},
  publisher={Elsevier}
}
@article{cazalilla1998theory,
  title={Theory of {A}uger neutralization and deexcitation of slow ions at metal surfaces},
  author={Cazalilla, MA and Lorente, Nicol{\'a}s and Muino, R Diez and Gauyacq, J-P and Teillet-Billy, D and Echenique, PM},
  journal={Phys. Rev. B},
  volume={58},
  number={20},
  pages={13991},
  year={1998},
  publisher={APS}
}
@article{auth1995high,
  title={High fractions of negative ions in grazing scattering of fast oxygen atoms from a {LiF}(100) surface},
  author={Auth, C and Borisov, AG and Winter, H},
  journal={Phys. Rev. Lett},
  volume={75},
  number={12},
  pages={2292},
  year={1995},
  publisher={APS}
}
@article{winter1996complete,
  title={Complete negative-ion conversion of halogen atoms and positive ions in surface scattering from {KI}(100)},
  author={Winter, H and Mertens, A and Auth, C and Borisov, AG},
  journal={Phys. Rev. A},
  volume={54},
  number={3},
  pages={2486},
  year={1996},
  publisher={APS}
}

@article{pan2021polar,
  title={Polar inelastic profiles in fast-atom diffraction at surfaces},
  author={Pan, Peng and Debiossac, Maxime and Roncin, Philippe},
  journal={Physical Review B},
  volume={104},
  number={16},
  pages={165415},
  year={2021},
  doi={10.1103/PhysRevB.104.165415},
  publisher={APS}
}
@article{pan2023lateral,
  title={Lateral line profiles in fast-atom diffraction at surfaces},
  author={Pan, Peng and Kanitz, Carina and Debiossac, Maxime and Le-Guen, Alex and Rad, Jaafar Najafi and Roncin, Philippe},
  journal={Phys. Rev. B},
  volume={108},
  number={3},
  pages={035413},
  year={2023},
  doi={10.1103/PhysRevB.108.035413},
  publisher={APS}
}
@article{wyputta1991h,
  title={H$^-$ formation in grazing collisions of fast protons with an {Al} (111) surface},
  author={Wyputta, F and Zimny, R and Winter, H},
  journal={NIM-B},
  volume={58},
  number={3-4},
  pages={379--383},
  year={1991},
  publisher={Elsevier}
}
@article{winter1992image,
  title={Image charge acceleration of multi-charged argon ions in grazing collisions with an aluminum surface},
  author={Winter, H},
  journal={E.P.L.},
  volume={18},
  number={3},
  pages={207},
  year={1992},
  publisher={IOP Publishing}
}//EuroPhysics Letters
@article{schuller2009fast,
  title={Fast atom diffraction from superstructures on a {Fe (110)} surface},
  author={Sch{\"u}ller, A and Busch, M and Wethekam, S and Winter, H},
  journal={Physical Review Letters},
  volume={102},
  number={1},
  pages={017602},
  year={2009},
  publisher={APS},
DOI = {10.1103/PhysRevLett.102.017602}
}
@article{winter1993image,
  title={Image acceleration of highly charged xenon ions in front of a metal surface},
  author={Winter, H and Auth, Ch and Schuch, R and Beebe, E},
  journal={Phys. Rev. Lett},
  volume={71},
  number={12},
  pages={1939},
  year={1993},
  publisher={APS},
 DOI = {10.1103/PhysRevLett.71.1939}
}
@article{igel1996intensity,
  title={Intensity oscillations in grazing scattering of fast {He}$^+$ ions during heteroepitaxial growth of {Cr on Fe} (100)},
  author={Igel, T and Pfandzelter, R and Winter, H},
  journal={Europhysics Letters},
  volume={35},
  number={1},
  pages={67},
  year={1996},
  publisher={IOP Publishing}
}
@article{borisov1998finite,
  title={Finite time effect in the charge transfer process during an ion-metal surface collision},
  author={Borisov, AG and Kazansky, AK and Gauyacq, JP},
  journal={Phys. Rev. Lett},
  volume={80},
  number={9},
  pages={1996},
  year={1998},
  publisher={APS},
 doi = {10.1103/PhysRevLett.80.1996}
}
@article{gadzuk1983vibrational,
  title={Vibrational excitation in molecule--surface collisions due to temporary negative molecular ion formation},
  author={Gadzuk, JW},
  journal={J. Chem. Phys.},
  volume={79},
  number={12},
  pages={6341--6348},
  year={1983},
  publisher={American Institute of Physics}
}
@article{oen1983shadow,
  title={Universal shadow cone expressions for an atom in an ion beam},
  author={Oen, Ordean S},
  journal={Surf. Sci. Lett},
  volume={131},
  pages={L407--L411},
  year={1983},
  publisher={Elsevier}
}%number={2-3},
@article{esaulov1994autoionising,
  title={Autoionising state excitation in collisions of inert gas projectiles with an {Al} surface and effects of initial stages of oxidation},
  author={Esaulov, VA and Guillemot, L and Lacombe, S},
  journal={NIM-B},
  volume={90},
  number={1-4},
  pages={305--309},
  year={1994},
  publisher={Elsevier}
}
@article{lakits1990threshold,
  title={Threshold of ion-induced kinetic electron emission from a clean metal surface},
  author={Lakits, G and Aumayr, F and Heim, M and Winter, HP},
  journal={Phys. Rev. A},
  volume={42},
  number={9},
  pages={5780},
  year={1990},
  publisher={APS}
}
@article{hayderer1999highly,
  title={A highly sensitive quartz-crystal microbalance for sputtering investigations in slow ion--surface collisions},
  author={Hayderer, G and Schmid, M and Varga, P and Winter, HP and Aumayr, F},
  journal={Rev. Sci. Instrum.},
  volume={70},
  number={9},
  pages={3696--3700},
  year={1999},
  publisher={American Institute of Physics}
}
@article{roncin2020revisiting,
  title={Revisiting atomic collisions physics with highly charged ions, a tribute to {Michel Barat}},
  author={Roncin, Philippe},
  journal={J. Phys. B},
  volume={53},
  number={20},
  pages={202001},
  year={2020},
  doi={10.1088/1361-6455/abaaf9},
  publisher={IOP Publishing}
}
@article{los1990charge,
  title={Charge exchange in atom-surface collisions},
  author={Los, Joop and Geerlings, Jacobus Johannes Cornelis},
  journal={Physics reports},
  volume={190},
  number={3},
  pages={133--190},
  year={1990},
  publisher={Elsevier}
}
@article{roncin1990observation,
  title={Observation of orientation propensity for electron capture in multiply-charged-ion--atom collisions},
  author={Roncin, P and Adjouri, C and Gaboriaud, MN and Guillemot, L and Barat, M and Andersen, N},
  journal={Phys. Rev. Lett},
  volume={65},
  number={26},
  pages={3261},
  year={1990},
doi={10.1103/PhysRevLett.65.3261},
  publisher={APS}
}
@article{Ullrich_1988,
Author = {ULLRICH, J and SCHMIDTBOCKING, H and KELBCH, C},
Title = {DETERMINATION OF VERY SMALL PROJECTILE SCATTERING ANGLES BY MEASURING
   RECOIL-ION TRANSVERSE VELOCITIES},
Journal = {NIM-A},
Year = {1988},
Volume = {268},
Number = {1},
Pages = {216-224},
Month = {MAY 10},
DOI = {10.1016/0168-9002(88)90610-9},
ISSN = {0168-9002},
Unique-ID = {WOS:A1988N314100026},
}
@article{roncin1999_Oq,
  title={Energy loss and secondary electron measurements in collisions at grazing angle of 10 {keV} {O}$^{q+}$ ions on LiF surface},
  author={Roncin, P and Barat, M and Atanas, JP and Villette, J and Morozov, V},
  journal={Phys. Scr.},
  volume={1999},
  number={T80B},
  pages={231},
  year={1999},
  publisher={IOP Publishing}
}
@article{ullrich1997recoil,
  title={Recoil-ion momentum spectroscopy},
  author={Ullrich, Joachim and Moshammer, Robert and D{\"o}rner, Reinhard and Jagutzki, Ottmar and Mergel, Volker and Schmidt-B{\"o}cking, Horst and Spielberger, Lutz},
  journal={J. Phys. B.},
  volume={30},
  number={13},
  pages={2917},
  year={1997},
  publisher={IOP Publishing}
}
@article{moshammer_1996_4pi,
  title={A 4$\pi$ recoil-ion electron momentum analyzer: a high-resolution “microscope” for the investigation of the dynamics of atomic, molecular and nuclear reactions},
  author={Moshammer, Robert and Unverzagt, M and Schmitt, W and Ullrich, J and Schmidt-B{\"o}cking, H},
  journal={NIM-B},
  volume={108},
  number={4},
  pages={425--445},
  year={1996},
  publisher={Elsevier}
}
@article{dorner2000cold,
  title={Cold target recoil ion momentum spectroscopy: a ‘momentum microscope' to view atomic collision dynamics},
  author={D{\"o}rner, Reinhard and Mergel, Volker and Jagutzki, Ottmar and Spielberger, Lutz and Ullrich, Joachim and Moshammer, Robert and Schmidt-B{\"o}cking, Horst},
  journal={Physics Reports},
  volume={330},
  number={2-3},
  pages={95--192},
  year={2000},
  publisher={Elsevier}
}
@article{chetioui1990doubly,
  title={Doubly excited states populated in collisions of {O}$^{8+}$ ions with {He} and {H}$_2$ at 1.24 {keV} amu$^{-1}$},
  author={Chetioui, A and Martin, F and Politis, MF and Rozet, JP and Touati, A and Blumenfeld, L and Vernhet, D and Wohrer, K and Stephan, C and Barat, M and others},
  journal={J. Phys. B},
  volume={23},
  number={20},
  pages={3659},
  year={1990},
  publisher={IOP Publishing}
}
@article{ostrovsky1991mechanisms,
  title={On the mechanisms for creation of the electron orbital polarization in the charge exchange processes},
  author={Ostrovsky, VN},
  journal={J. Phys. B},
  volume={24},
  number={20},
  pages={L507},
  year={1991},
  publisher={IOP Publishing}
}
@article{adjouri1994quasimolecular,
  title={Quasimolecular analysis of orientation and alignment in {B}$^{3+}$-rare gas electron capture processes},
  author={Adjouri, C and Roncin, P and Gaboriaud, MN and Barat, M and Andersen, N},
  journal={J. Phys. B},
  volume={27},
  number={14},
  pages={3093},
  year={1994},
  doi={10.1088/0953-4075/27/14/041},
  publisher={IOP Publishing}
}
@article{armand_1982_scattering,
  title={Scattering of neutral particles by an exponential corrugated potential: A solution for high corrugation amplitude},
  author={Armand, G and Manson, JR},
  journal={Phys. Rev. B},
  volume={25},
  number={10},
  pages={6195},
  year={1982},
  publisher={APS}
}

@article{gravielle_2014_semiquantum,
  title={Semiquantum approach for fast atom diffraction: Solving the rainbow divergence},
  author={Gravielle, Maria Silvia and Miraglia, Jorge Esteban},
  journal={Phys. Rev. A},
  volume={90},
  number={5},
  pages={052718},
  year={2014},
  publisher={APS}
}

@article{schuller_2009_he,
  title={{He-LiF} surface interaction potential from fast atom diffraction},
  author={Sch{\"u}ller, A and Winter, H and Gravielle, Maria Silvia and Pruneda, JM and Miraglia, Jorge Esteban},
  journal={Phys. Rev. A},
  volume={80},
  number={6},
  pages={062903},
  year={2009},
  publisher={APS}
}

@article{schuller_NIMB_2009,
  title={Diffraction of fast atoms under axial surface channeling conditions},
  author={Sch{\"u}ller, A and Winter, H},
  journal={NIM-B},
  volume={267},
  number={4},
  pages={628--633},
  year={2009},
  publisher={Elsevier},
  doi={10.1016/j.nimb.2008.11.052}
}
